Guaranteed-Safe Approximate Reachability via State Dependency-Based Decomposition

Hamilton Jacobi (HJ) Reachability is a formal verification tool widely used in robotic safety analysis. Given a target set as unsafe states, a dynamical system is guaranteed not to enter the target under the worst-case disturbance if it avoids the Backward Reachable Tube (BRT). However, computing BRTs suffers from exponential computational time and space complexity with respect to the state dimension. Previously, system decomposition and projection techniques have been investigated, but the trade off between applicability to a wider class of dynamics and degree of conservatism has been challenging. In this paper, we propose a State Dependency Graph to represent the system dynamics, and decompose the full system where only dependent states are included in each subsystem, and "missing" states are treated as bounded disturbance. Thus for a large variety of dynamics in robotics, BRTs can be quickly approximated in lower-dimensional chained subsystems with the guaranteed-safety property preserved. We demonstrate our method with numerical experiments on the 4D Quadruple Integrator, and the 6D Bicycle, an important car model that was formerly intractable.

==> sections/future_work.tex <==
% \section{Future work}
% To compute reach set, we need inner approximation in projection.

% If we can compute reach set, we can somehow overcome share control problem, 


==> sections/picture.tex <==
\section{picture}
%%%%%%%%%%%%%%%try picture%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}

% \begin{picture}(0,0)

% \put(10,5){\includegraphics[scale=0.08]{figures/opt_traj/com1/one.png}}

% \put(90,5){\includegraphics[scale=0.08]{figures/opt_traj/com1/two.png}}

% \put(170,5){\includegraphics[scale=0.08]{figures/opt_traj/com1/three.png}}

% \put(250,5){\includegraphics[scale=0.08]{figures/opt_traj/com1/four.png}}

% \put(330,5){\includegraphics[scale=0.08]{figures/opt_traj/com1/five.png}}

% \put(410,5){\includegraphics[scale=0.08]{figures/opt_traj/com1/six.png}}

% \end{picture}
% \caption{This is some figure side by side}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!htb]
  \centering
  \begin{subfigure}{.20\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com1/t00.png}
  \end{subfigure}%
  \hspace{0.1pt}% Space between image A and B
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com1/t04.png}
  \end{subfigure}%
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com1/t08.png}
  \end{subfigure}
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com1/t12.png}
  \end{subfigure}
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com1/t16.png}
  \end{subfigure}
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com1/t20.png}
  \end{subfigure}
  \caption{A number of images}
\end{figure*}

\begin{figure*}[!htb]
  \centering
  \begin{subfigure}{.20\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com2/t00.png}
  \end{subfigure}%
  \hspace{0.1pt}% Space between image A and B
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com2/t04.png}
  \end{subfigure}%
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com2/t08.png}
  \end{subfigure}
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com2/t12.png}
  \end{subfigure}
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com2/t16.png}
  \end{subfigure}
  \hspace{0.1pt}% Space between image B and C
  \begin{subfigure}{.15\linewidth}
    \centering
    \includegraphics[width = \linewidth]{figures/opt_traj/com2/t20.png}
  \end{subfigure}
  \caption{A number of images}
\end{figure*}

==> sections/prob_formulation.tex <==
% \section{Problem formulation} \label{sec:formulation}
% %This part only takes 1/3 columns

% {\color{red}
% How should we define the problem?
% }

% Given the target set $\mathcal{T}$ as obstacles, and the full system dynamics in (1),
% \begin{equation*}
%     S(x, f, u, d): x = (x_{1}, x_{2}, x_{3}, x_{4})
% \end{equation*}
% with dynamics in [], 

% we'd like to decompose S into several lower-dimension subsystem.
